A Euclidean Signature Semi-Classical Program

In this article we discuss our ongoing program to extend the scope of certain, well-developed microlocal methods for the asymptotic solution of Schr\"{o}dinger's equation (for suitable `nonlinear oscillatory' quantum mechanical systems) to the treatment of several physically significant, interacting quantum field theories. Our main focus is on applying these `Euclidean-signature semi-classical' methods to self-interacting (real) scalar fields of renormalizable type in 2, 3 and 4 spacetime dimensions and to Yang-Mills fields in 3 and 4 spacetime dimensions. A central argument in favor of our program is that the asymptotic methods for Schr\"{o}dinger operators developed in the microlocal literature are far superior, for the quantum mechanical systems to which they naturally apply, to the conventional WKB methods of the physics literature and that these methods can be modified, by techniques drawn from the calculus of variations and the analysis of elliptic boundary value problems, to apply to certain (bosonic) quantum field theories. Unlike conventional (Rayleigh/ Schr\"{o}dinger) perturbation theory these methods allow one to avoid the artificial decomposition of an interacting system into an approximating `unperturbed' system and its perturbation and instead to keep the nonlinearities (and, if present gauge invariances) of an interacting system intact at every level of the analysis.

==> sec-finite_dim.tex <==
\section{Modified Semi-Classical Methods for finite dimensional problems}
\label{sec:finite_dim}

\subsection{An application to Nonlinear Quantum Oscillations Problems}
\label{subsec:qm}
\cite{Moncrief:2012}

\subsection{Homogeneous cosmology results for the Wheeler-DeWitt equation}
\label{subsec:cosmo_w-dw}

\subsection{An application to Supersymmetric Quantum Mechanics}
\label{subsec:susy_qm}

